Euclid Quick Data Release (Q1). Searching for radio-selected \Euclid-dark galaxies in the EDF-N

We present and investigate the properties of a sample of radio-selected, Euclid-dark galaxies, identified from LOFAR HBA observations at 144 MHz within the Euclid Deep Field-North (EDF-N). Starting from radio sources lacking optical counterparts in previous surveys, but detected with Spitzer/IRAC, we identified 166 galaxies with no emission at a more than $3\sigma$ level in Euclid Quick Release 1 (Q1) images, and no matches in the Euclid Q1 catalogue. To minimise contamination from nearby sources, we selected a sub-sample of 88 isolated galaxies. By exploiting multi-band images and catalogues available for the EDF-N, we inferred the physical properties of our sample via SED fitting. The resulting redshift distribution spans $0.4 \leq z_\mathrm{ph} \leq 5.0$. We used recent sub-arcsecond imaging from the International LOFAR Telescope to constrain the nature of the compact radio emission through brightness temperature estimates. By combining this information with the radio excess relative to the infrared/radio correlation (IRRC), we searched for possible active galactic nuclei (AGN) activity. Approximately 40% of our sources show evidence of AGN activity. The Euclid-dark sources detected in the far-infrared are consistent with a population of heavily obscured, massive star-forming galaxies with high star formation rates. Their location above the star-forming main sequence is consistent with similar near-infrared-dark galaxy populations reported in the literature. We also performed a UV-to-radio median stacking analysis, finding that the two subsamples exhibit similar global physical properties and differ primarily in their radio emission. These preliminary results indicate that the wide area covered by Euclid enables the identification of a higher fraction of systems in which intense star formation and AGN activity coexist, likely capturing a key phase of galaxy--black hole co-evolution.

==> Tables/TableB1_short.tex <==
\begin{tabular}{ccccccccccc}
\hline
\hline
\noalign{\vskip 2pt}
  \multicolumn{1}{c}{ID} &
  \multicolumn{1}{c}{RA [deg]} &
  \multicolumn{1}{c}{Dec [deg]} &
  \multicolumn{1}{c}{$z$} &
  \multicolumn{1}{c}{$\sigma_{z}$} &
  \multicolumn{1}{c}{$M_{\rm UV}$} &
  \multicolumn{1}{c}{$\sigma_{M_{\rm UV}}$} &
  \multicolumn{1}{c}{$\beta_{\rm UV}$} &
  \multicolumn{1}{c}{$\sigma_{\beta_{\rm UV}}$} &
  \multicolumn{1}{c}{$\beta_{\rm opt}$} &
  \multicolumn{1}{c}{$\sigma_{\beta_{\rm opt}}$} \\
\hline
\noalign{\vskip 2pt}
  $-508115529279019500$ & 50.811552 & $-27.901950$ & 1.73 & 0.04 & $-19.3$ & 0.4 & $-2.5$ & 0.8 & 1.3 & 0.7\\
  $-509746984272137369$ & 50.974698 & $-27.213736$ & 1.43 & 0.01 & $-19.1$ & 0.4 & $-2.3$ & 0.6 & 0.4 & 0.4\\
  $-506780226277952382$ & 50.678022 & $-27.795238$ & 1.84 & 0.09 & $-19.2$ & 0.2 & $-2.0$ & 0.5 & 1.0 & 0.5\\
  $-508524594269841903$ & 50.852459 & $-26.984190$ & 2.08 & 0.05 & $-19.4$ & 0.2 & $-1.2$ & 0.5 & 0.2 & 0.7\\
  $-508984186271393227$ & 50.898418 & $-27.139322$ & 2.04 & 0.01 & $-19.1$ & 0.4 & $-1.3$ & 0.7 & 0.8 & 0.9\\
  $-509604641270953419$ & 50.960464 & $-27.095341$ & 1.56 & 0.07 & $-18.5$ & 0.5 & $-1.7$ & 0.8 & 0.8 & 0.5\\
  $-508222098269760365$ & 50.822209 & $-26.976036$ & 1.93 & 0.02 & $-19.6$ & 0.2 & $-1.5$ & 0.4 & 0.2 & 0.5\\
  $-508762123270516640$ & 50.876212 & $-27.051664$ & 1.56 & 0.01 & $-19.4$ & 0.3 & $-2.6$ & 0.6 & 0.1 & 0.5\\
  $-508397504271496709$ & 50.839750 & $-27.149670$ & 2.04 & 0.07 & $-19.1$ & 0.4 & $-1.8$ & 0.9 & 1.4 & 1.2\\
  $-509723625268249072$ & 50.972362 & $-26.824907$ & 1.67 & 0.19 & $-18.4$ & 0.5 & $-1.3$ & 0.6 & 0.4 & 0.6\\
  \hline
\end{tabular}
